Unconditional finite amplitude stability of a viscoelastic fluid in a mechanically isolated vessel with spatially non-uniform wall temperature

We investigate finite amplitude stability of spatially inhomogeneous steady state of an incompressible viscoelastic fluid which occupies a mechanically isolated vessel with walls kept at spatially non-uniform temperature. For a wide class of incompressible viscoelastic models including the Oldroyd-B model, the Giesekus model, the FENE-P model, the Johnson--Segalman model, and the Phan--Thien--Tanner model we prove that the steady state is stable subject to any finite perturbation.

==> vit-prusa-env-list.tex <==
% theorems, remarks, definitions, etc.
% requires amsmath, amsthm

\newtheorem{theorem}{Theorem} % this must be commented out if we use \usepackage{thmtools}

%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Lemma}

%\theoremstyle{corollary}
\newtheorem{corollary}[theorem]{Corollary}

%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition} % this must be commented out if we use \usepackage{thmtools}

\theoremstyle{proposition}
\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{assumption}
%\newtheorem{assumption}[theorem]{Assumption} 
%\theoremstyle{condition}
%\newtheorem{condition}[theorem]{Condition} 

\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{problem}[theorem]{Problem} 

%\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}


==> vit-prusa-macros-reference-natural.tex <==
\newcommand{\rplacer}{\kappa_0}       % placer, reference configuration
\newcommand{\cplacer}{\kappa_t}       % placer, current configuration
\newcommand{\nplacer}{\kappa_{\mathnormal{p}(\mathnormal{t})}}  % placer, natural configuration

\newcommand{\refnat}{\mathrm{RN}} % reference -> natural
\newcommand{\natcur}{\mathrm{NC}} % natural -> current
\newcommand{\refcur}{\mathrm{RC}} % reference -> current

% PRUSA
% \newcommand{\fgradrn}{\ensuremath{\fgrad_{\refnat}}} % deformation gradient, reference -> natural
% \newcommand{\fgradrng}{\ensuremath{\fgrad_{\refnat}}} % deformation gradient, reference -> natural, symbol G

% \newcommand{\gradvlrn}{\ensuremath{\gradvl_{\refnat}}} % velocity gradient, reference -> natural
% \newcommand{\gradsymrn}{\ensuremath{\gradsym_{\refnat}}} % symmetric part of the velocity gradient, reference -> natural
% \newcommand{\gradasymrn}{\ensuremath{\gradasym_{\refnat}}} % skew symmetric part of the velocity gradient, reference -> natural
% \newcommand{\lcgnc}{\ensuremath{\lcg_{\natcur}}} % left Cauchy--Green tensor, natural -> current
% \newcommand{\rcgnc}{\ensuremath{\rcg_{\natcur}}} % right Cauchy--Green tensor, natural -> current

% \newcommand{\fgradnc}{\ensuremath{\fgrad_{\natcur}}} % deformation gradient, natural -> current
% \newcommand{\fgradrc}{\ensuremath{\fgrad_{\refcur}}} % deformation gradient, reference -> current


% MALEK
\newcommand{\fgradrn}{\ensuremath{\fgrad_{\rplacer(\body)\to \nplacer(\body)}}} % deformation gradient, reference -> natural
\newcommand{\fgradrng}{\ensuremath{\tensorq{G}}} % deformation gradient, reference -> natural, symbol G

\newcommand{\gradvlrn}{\ensuremath{\gradvl_{\nplacer}}} % velocity gradient, reference -> natural
\newcommand{\gradsymrn}{\ensuremath{\gradsym_{\nplacer}}} % symmetric part of the velocity gradient, reference -> natural
\newcommand{\gradasymrn}{\ensuremath{\gradasym_{\nplacer}}} % skew symmetric part of the velocity gradient, reference -> natural

\newcommand{\lcgnc}{\ensuremath{\lcg_{\nplacer}}} % left Cauchy--Green tensor, natural -> current
\newcommand{\lcgncc}{\ensuremath{\lcgc_{\nplacer}}} % left Cauchy--Green tensor, natural -> current, components

\newcommand{\rcgnc}{\ensuremath{\rcg_{\nplacer}}} % right Cauchy--Green tensor, natural -> current
\newcommand{\rcgncc}{\ensuremath{\rcgc_{\nplacer}}} % right Cauchy--Green tensor, natural -> current, components

\newcommand{\fgradnc}{\ensuremath{\fgrad_{\nplacer}}} % deformation gradient, natural -> current
\newcommand{\fgradrc}{\ensuremath{\fgrad}} % deformation gradient, reference -> current, components
